Cantor meets Scott: Semantic Foundations for Probabilistic Networks

ProbNetKAT is a probabilistic extension of NetKAT with a denotational semantics based on Markov kernels. The language is expressive enough to generate continuous distributions, which raises the question of how to compute effectively in the language. This paper gives an new characterization of ProbNetKAT's semantics using domain theory, which provides the foundation needed to build a practical implementation. We show how to use the semantics to approximate the behavior of arbitrary ProbNetKAT programs using distributions with finite support. We develop a prototype implementation and show how to use it to solve a variety of problems including characterizing the expected congestion induced by different routing schemes and reasoning probabilistically about reachability in a network.

==> figures/4cycle.tex <==

\begin{framedfigure*}
\tikzset{
  switch/.style={
    circle,
    fill=black!25,
    draw=black!50,
    very thick,
    minimum size=20pt,
    inner sep=0pt},
  host/.style={
    rectangle,
    fill=black!25,
    draw=black!50,
    very thick,
    minimum size=14pt,
    inner sep=0pt},
}

\begin{minipage}{.32\textwidth}
\smallskip
\noindent
\centerline{\begin{tikzpicture}
    \node[switch] (S1) {\textsf{S1}};
    \node[switch] (S2) [right = 1cm  of S1]  {\textsf{S2}};
    \node[switch] (S3) [below = 1cm  of S2] {\textsf{S3}};
    \node[switch] (S4) [below = 1cm  of S1] {\textsf{S4}};
    \node[host] (H1) [above left  = 0.5cm of S1] {\textsf{h1}};
    \node[host] (H2) [above right = 0.5cm of S2] {\textsf{h2}};
    \node[host] (H3) [below right = 0.5cm of S3] {\textsf{h3}};
    \node[host] (H4) [below left  = 0.5cm of S4] {\textsf{h4}};
    \path[draw]
    (S1) edge node [above,pos=0.1] {\small \sf 1} (H1)
    (S2) edge node [above,pos=0.1] {\small \sf 2} (H2)
    (S3) edge node [below,pos=0.1] {\small \sf 3} (H3)
    (S4) edge node [below,pos=0.1] {\small \sf 4} (H4)
    (S1) edge node [above,pos=0.1] {\small \sf 2} node [above,pos=0.9] {\small \sf 1} (S2)
    (S2) edge node [right,pos=0.1] {\small \sf 3} node [right,pos=0.9] {\small \sf 2} (S3)
    (S3) edge node [below,pos=0.1] {\small \sf 4} node [below,pos=0.9] {\small \sf 3} (S4)
    (S4) edge node [left ,pos=0.1] {\small \sf 1} node [left ,pos=0.9] {\small \sf 4} (S1);
\end{tikzpicture}}
\centerline{\small (a)}
\end{minipage}\vrule\begin{minipage}{.333\textwidth}
\noindent
\centerline{\tikz\node{\pgfimage[width=.97\textwidth]{"figures/15iter/4cycle_intro/Max Congestion-line"}};}
\centerline{\small (b)}
\end{minipage}\vrule\begin{minipage}{.34\textwidth}
\noindent
\centerline{\tikz\node{\pgfimage[width=.97\textwidth]{"figures/15iter/4cycle_intro_break_1_2/Throughput-bar"}};}
\centerline{\small (c)}
\end{minipage}
\caption{(a) topology, (b) max congestion under no failure, (c) throughput when
$S_1 \rightarrow S_2$ link breaks SPF routes all 2-hop traffic clockwise.
Demand between every pair of nodes is 1/8. h1 to h3 has demand 1/2. Under no
failure: in case of SPF, one of the max congested links $(S1 \rightarrow S2)$
carries traffic for $h1 \rightarrow h2$, $h4 \rightarrow h2$, $h1 \rightarrow
h3$ leading to $\frac{1}{8} + \frac{1}{8} + \frac{1}{2} = \frac{3}{4} = 0.75$ units of
traffic. Since every link has unit capacity, max congestion = 0.75. In case of ECMP, $(S1 \rightarrow S2)$ is still one of the max
congested links, carrying traffic for $h1 \rightarrow h2$, $\frac{1}{2} ~h4
\rightarrow h2$, $\frac{1}{2} ~h1 \rightarrow h3$ = $\frac{1}{8} + \frac{1}{16}
+ \frac{1}{4} \approx 0.43$. Throughput: Under no failure, both have throughput 1.
Aggregate demand = $\frac{1}{8} \times 3 \times 3 + (\frac{1}{8} +\frac{1}{8}
+\frac{1}{2}) = \frac{15}{8}$. In case of failure: SPF loses $\frac{3}{4}$
units. So, tput = $\frac{15}{8} - \frac{3}{4} = \frac{9}{8}$ which is
$60\%$. ECMP loses $\frac{7}{16}$
units. So, tput = $\frac{15}{8} - \frac{7}{16} = \frac{23}{16}$ which is $77\%$.}
\label{fig:4cycle}
\end{framedfigure*}




==> figures/ecmp_pnk.tex <==

\input{./figures/4cycle.tex}

ProbNetKAT term for ECMP based routing in 4-cycle topology:
\[
  \begin{array}{r@{\quad}l}
    & (\pseq{\pseq{\match{sw}{S_1}}{\match{dst}{h_1}}}{\modify{pt}{0}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_1}}{\match{dst}{h_2}}}{\modify{pt}{2}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_1}}{\match{dst}{h_3}}}{(\modify{pt}{4} \oplus_{0.5} \modify{pt}{2})}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_1}}{\match{dst}{h_4}}}{\modify{pt}{4}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_2}}{\match{dst}{h_1}}}{\modify{pt}{1}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_2}}{\match{dst}{h_2}}}{\modify{pt}{0}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_2}}{\match{dst}{h_3}}}{\modify{pt}{3}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_2}}{\match{dst}{h_4}}}{(\modify{pt}{3} \oplus_{0.5} \modify{pt}{1})}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_3}}{\match{dst}{h_1}}}{(\modify{pt}{4} \oplus_{0.5} \modify{pt}{2})}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_3}}{\match{dst}{h_2}}}{\modify{pt}{2}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_3}}{\match{dst}{h_3}}}{\modify{pt}{0}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_3}}{\match{dst}{h_4}}}{\modify{pt}{4}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_4}}{\match{dst}{h_1}}}{\modify{pt}{1}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_4}}{\match{dst}{h_2}}}{(\modify{pt}{3} \oplus_{0.5} \modify{pt}{1})}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_4}}{\match{dst}{h_3}}}{\modify{pt}{3}}) \\
    \pcomp & (\pseq{\pseq{\match{sw}{S_4}}{\match{dst}{h_4}}}{\modify{pt}{0}})
  \end{array}
\]

